WiseAD: Knowledge Augmented End-to-End Autonomous Driving with Vision-Language Model

The emergence of general human knowledge and impressive logical reasoning capacity in rapidly progressed vision-language models (VLMs) have driven increasing interest in applying VLMs to high-level autonomous driving tasks, such as scene understanding and decision-making. However, an in-depth study on the relationship between knowledge proficiency, especially essential driving expertise, and closed-loop autonomous driving performance requires further exploration. In this paper, we investigate the effects of the depth and breadth of fundamental driving knowledge on closed-loop trajectory planning and introduce WiseAD, a specialized VLM tailored for end-to-end autonomous driving capable of driving reasoning, action justification, object recognition, risk analysis, driving suggestions, and trajectory planning across diverse scenarios. We employ joint training on driving knowledge and planning datasets, enabling the model to perform knowledge-aligned trajectory planning accordingly. Extensive experiments indicate that as the diversity of driving knowledge extends, critical accidents are notably reduced, contributing 11.9% and 12.4% improvements in the driving score and route completion on the Carla closed-loop evaluations, achieving state-of-the-art performance. Moreover, WiseAD also demonstrates remarkable performance in knowledge evaluations on both in-domain and out-of-domain datasets.

==> sec/final_copy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/teaser.tex <==
% \begin{figure*}[!h]
% \centering
% % \includegraphics[width=0.5\textwidth %height=0.5\textwidth
% % ]{figs}
% \includegraphics[width=0.8\textwidth]{figs/teaser.pdf}
% \caption{\textbf{An overview of our \OURS}, a specialized vision-language model for end-to-end autonomous driving with extensive fundamental driving knowledge. Given a clip of the video sequence, our \OURS is capable of answering various driving-related questions and planning a trajectory according to the target waypoint.}
% \label{fig:teaser}
% \end{figure*}



==> tables/joint_training.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{Ablation studies on different training recipes.}\label{tab:training_recipe}
%     \vspace{1mm}
%     \setlength\tabcolsep{4pt}
%     \renewcommand\arraystretch{1.2}
%     \begin{tabular}{c|c|c|c|c|c|c|c} \hline
%     \multirow{2}{*}{Datasets} & \multirow{2}{*}{Pretrained Model} & \multicolumn{5}{c|}{Carla Closed-Loop Eval} & LingoQA Eval \\ \cline{3-8} 
%     & & DS $\uparrow$ & RC $\uparrow$ & IS $\uparrow$ & Red Light $\downarrow$ & Collisions $\downarrow$ & Lingo-Judge$\uparrow$ \\ \hline
%     \multicolumn{8}{c}{Sequential Training} \\ \hline
%     C & MobileVLM-1.7B & 62.46 & 83.47 &\textbf{ 0.74} & 8 & 12 & 13.4 \\ \hline
%     C & LingoQA-Pretrained & 52.30 & 75.11 & 0.71 & 10 & 16 & 12.8 \\ \hline
%     \multicolumn{8}{c}{Joint Training} \\ \hline
%     C+L & MobileVLM-1.7B & \textbf{63.80} & \textbf{87.96} & 0.72 & 9 & \textbf{12} & \textbf{58.2} \\ \hline
%     % \multicolumn{8}{c}{\OURS-7B} \\ \hline
%     \end{tabular}
%     % \begin{tabular}{c|c|c|c|c|c} \hline
%     % \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{HPatches} & \multicolumn{2}{c|}{ETH3D} & KITTI \\ \cline{2-6}
%     % & AEPE & PCK-1 & AEPE & PCK-1 & F1\\ \hline
%     % C+T & 55.3 & 38.3 & 3.9 & 55.0 & 13.9 \\ \hline
%     % M & 24.9 & 44.8  & 2.2 & 50.6 & 18.4 \\ \hline
%     % M+Sc & 15.3 & 42.8 & \textbf{2.0} & 54.1 & 17.7\\ \hline
%     % M+Sc+T+TA & \textbf{13.1} & 44.3 & \textbf{2.0} & 55.9 & 10.8  \\ \hline
%     % M+Sc+T+TA+TS & 13.3 & \textbf{46.3}  & \textbf{2.0} & \textbf{56.3} & \textbf{9.6} \\ \hline
%     % \end{tabular}
% \end{table*}
% \vspace{-1mm}



% \begin{table*}[h]
%     \centering
%     \caption{Ablation studies on different training recipes.}\label{tab:training_recipe}
%     \vspace{1mm}
%     \setlength\tabcolsep{4pt}
%     \renewcommand\arraystretch{1.2}
%     \begin{tabular}{c|c|c|c|c|c|c|c} \hline
%     \multirow{2}{*}{Datasets} & \multirow{2}{*}{Pretrained Model} & \multicolumn{5}{c|}{Carla Closed-Loop Eval} & LingoQA Eval \\ \cline{3-8} 
%     & & DS $\uparrow$ & RC $\uparrow$ & IS $\uparrow$ & Red Light $\downarrow$ & Collisions $\downarrow$ & Lingo-Judge$\uparrow$ \\ \hline
%     \multicolumn{8}{c}{Sequential Training} \\ \hline
%     C & MobileVLM-1.7B & 62.46 & 83.47 &\textbf{ 0.74} & 8 & 12 & 13.4 \\ \hline
%     C & LingoQA-Pretrained & 52.30 & 75.11 & 0.71 & 10 & 16 & 12.8 \\ \hline
%     \multicolumn{8}{c}{Joint Training} \\ \hline
%     C+L & MobileVLM-1.7B & \textbf{63.80} & \textbf{87.96} & 0.72 & 9 & \textbf{12} & \textbf{58.2} \\ \hline
%     % \multicolumn{8}{c}{\OURS-7B} \\ \hline
%     \end{tabular}
%     % \begin{tabular}{c|c|c|c|c|c} \hline
%     % \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{HPatches} & \multicolumn{2}{c|}{ETH3D} & KITTI \\ \cline{2-6}
%     % & AEPE & PCK-1 & AEPE & PCK-1 & F1\\ \hline
%     % C+T & 55.3 & 38.3 & 3.9 & 55.0 & 13.9 \\ \hline
%     % M & 24.9 & 44.8  & 2.2 & 50.6 & 18.4 \\ \hline
%     % M+Sc & 15.3 & 42.8 & \textbf{2.0} & 54.1 & 17.7\\ \hline
%     % M+Sc+T+TA & \textbf{13.1} & 44.3 & \textbf{2.0} & 55.9 & 10.8  \\ \hline
%     % M+Sc+T+TA+TS & 13.3 & \textbf{46.3}  & \textbf{2.0} & \textbf{56.3} & \textbf{9.6} \\ \hline
%     % \end{tabular}
% \end{table*}
% \vspace{-1mm}
